Social Media Should Feel Like Minecraft, Not Instagram: Youth Visions for Meaningful Social Connections through Fictional Inquiry

We conducted co-design workshops with 23 participants (ages 15--24) to explore how youth envision ideal remote social connection. Using Fictional Inquiry (FI) within a Harry Potter-inspired narrative, we found that youth perceive a disconnect between platforms labeled ``social media'' (like Instagram) and those where they actually experience meaningful connections (like Minecraft or Discord). Participants envisioned an immersive platform prioritizing meaningful social connection through presence and immersion, natural self-expression, intuitive spatial navigation leveraging physical-world norms, and playful, low-stakes opportunities for friendship development. We synthesize these visions into six themes articulating relational needs that current platforms systematically marginalize. The FI method proved effective in generating innovative ideas while empowering youth by fostering hope and agency over social media's future. Our findings challenge ``doom'' narratives by reframing social media's harms as outcomes of specific design choices, demonstrating how design research can reopen space for imagining more supportive forms of mediated connection.

==> formatting/dev-commands.tex <==
%!TEX root = main.tex

%%
%% Note: This file includes all new commands that are needed for the preliminary 
%% paper-writing (draft / review) stage of the paper. These commands should NOT
%% be included in the camera-ready version of the paper.
%%
%% All content in this file should take at least one argument. Custom commands 
%% for simple aliases should be provided in "dev-aliases.tex".
%%

%% Note: Custom colors for in-paper comments
\definecolor{LIGHTPINK}{RGB}{237,157,202}
\definecolor{LIGHTRED}{RGB}{210,121,121}
\definecolor{LIGHTORANGE}{RGB}{230,170,50}
\definecolor{LIGHTGOLD}{RGB}{210,194,121}
\definecolor{LIGHTGREEN}{RGB}{121,210,121}
\definecolor{LIGHTAQUA}{RGB}{121,206,210}
\definecolor{LIGHTBLUE}{RGB}{121,124,210}
\definecolor{LIGHTPURPLE}{RGB}{153,102,255}
\definecolor{RED}{RGB}{178,34,34}
\definecolor{GRAY}{RGB}{166,166,166}
\definecolor{WHITE}{RGB}{255,255,255}

%% Note: General TODO and cut commands
\newcommand{\todo}[1]{
    \addcontentsline{toc}{subsection}{  %
        \protect\numberline{}           % Align text appropriately
        \textcolor{RED}{[TODO] #1}}     % Add todo to the table of contents
    \textcolor{RED}{[TODO] \emph{#1}}}  % Typeset the todo note in the text
\newcommand{\cut}[1]{\textcolor{RED}{\st{#1}}}
\newcommand{\revise}[1]{\textcolor{blue}{#1}}

%%
%% Note: Labeled in-paper comments for collaborators (with and without underlined
%% text). Each author should specify a new command for their name with a
%% different comment color, using the example new command for \jane below. 
%% Alternatively, authors can use the more complicated \guest command, but must
%% provide their name each time they leave a comment.
%%

%% Usage: \jane[(OPTIONAL) Text to underline in square brackets]{Comment.}
\newcommandx{\jane}[2][1=] 
    {\setulcolor{LIGHTGREEN}{\ul{#1}} \textcolor{LIGHTGREEN}
    {[\textbf{Jane:} #2]}}
%% Usage: \guest[(OPTIONAL) Text to underline]{Name}{Comment text}
\newcommandx{\guest}[3][1=]
    {\setulcolor{LIGHTORANGE}{\ul{#1}} \textcolor{LIGHTORANGE} 
    {[\textbf{#2:} #3]}}

%%
%% Note: Custom status badges can be added to sections and subsections to label 
%% which ones are ready (or not) for feedback to facilitate collaboration amongst
%% authors. Badges should be added directly to the section heading.
%%
\newcommand{\badge}[2]{\colorbox{#1}{\small\textcolor{WHITE}{\texttt{#2}}}}
\newcommand{\headerBadge}[2]{\hspace*{\fill}\badge{#1}{#2}}

\newcommand{\locked}{\headerBadge{LIGHTPURPLE}{locked}}
\newcommand{\complete}{\headerBadge{LIGHTBLUE}{complete}}
\newcommand{\feedbackProvided}{\headerBadge{LIGHTGREEN}{feedback provided}}
\newcommand{\readyForFeedback}{\headerBadge{LIGHTORANGE}{feedback requested}}
\newcommand{\underRevision}{\headerBadge{LIGHTRED}{under revision}}
\newcommand{\incomplete}{\headerBadge{RED}{incomplete}}



